Nonlinearity Compensation in a Multi-DoF Shoulder Sensing Exosuit for Real-Time Teleoperation

The compliant nature of soft wearable robots makes them ideal for complex multiple degrees of freedom (DoF) joints, but also introduce additional structural nonlinearities. Intuitive control of these wearable robots requires robust sensing to overcome the inherent nonlinearities. This paper presents a joint kinematics estimator for a bio-inspired multi-DoF shoulder exosuit capable of compensating the encountered nonlinearities. To overcome the nonlinearities and hysteresis inherent to the soft and compliant nature of the suit, we developed a deep learning-based method to map the sensor data to the joint space. The experimental results show that the new learning-based framework outperforms recent state-of-the-art methods by a large margin while achieving 12ms inference time using only a GPU-based edge-computing device. The effectiveness of our combined exosuit and learning framework is demonstrated through real-time teleoperation with a simulated NAO humanoid robot.

==> extraStuff.tex <==
\section{RESULTS AND DISCUSSION}
\label{sec:resAndDisc}

\subsection{Tendon-Routing Architecture Behaviour Analysis}
\label{subsec:fKinRes}

The behaviour of the tendon routing architecture conceptualized in Section \ref{sec:sysDes} is analyzed here. Fig.\ref{fig:arcLenvsAngles} presents the forward kinematics mapping ($\textbf{q}\mapsto\textbf{S}$) of the data from the 4 virtual sensors on moving the shoulder in 2 DoFs.  Fig.\ref{fig:arcLenvsAngles} shows $10\%$ of the sensor values (blue dots) and the ANN-fitted surface.  Analyzing this mapping is the first step to the actuation framework of the exosuit. This study is crucial as there are infinite tendon-routing combinations, and that even though the sensing tendons can sense during both extending/retracting, actuating tendons can only apply forces when pulling (monotonously decreasing). 

We can use the $\textbf{q}\mapsto\textbf{S}$ map (in Fig.\ref{fig:arcLenvsAngles}) to predict if the actuation tendons will displace monotonously and apply the required forces, if the same routing was used for actuation as well. The tendon-routing architecture analysis presented here was further required to isolate the source of the non-monotonous tendon displacement behaviour observed when the same analysis was performed on the simulation-based study presented in \cite{Varghese2019BSN}. We hypothesized two potential sources for the non-monotonicity: 1). a sub-optimal tendon-routing architecture, or 2). the limitation in OpenSim which only allowed for markers to be attached to the bones rather than on the skin surface, as would happen in reality. The hypothesis of the tendon-routing architecture being the error source is invalidated in this study.   


% Though the sensing map looks promising for actuation we are currently working on optimizing the tendon-routing to maximize tendon travel for the different movements experienced during ADL.

%  The mapping shown in Fig.\ref{fig:arcLenvsAngles} is the equivalent forward kinematics of the end-points of these sensors (on the upper-arm) in the tendon path-length space. This mapping is the resultant outcome of eq.\ref{eq:deltaarcLen}. 
From Fig.\ref{fig:arcLenvsAngles}, it can be seen that the sensors' behaviour match the behaviour of the equivalent muscles/synergies on which their paths are based. For \textit{e.g.}, it can be seen that during flexion, sensor value $\textbf{F}$ monotonously decreases and sensor value $\textbf{R}$ monotonously increases, and vice-versa during extension (see cyan and green line in Fig.\ref{fig:arcLenvsAngles}(a)\&(d)). This is consistent with the behaviour of the AD, PM, TM and LDo muscles on which tendons $\textbf{F}$ \& $\textbf{R}$ have been based. Similarly, during abduction, sensors-$\textbf{SF}$ and $\textbf{SR}$ monotonously decrease (see the magenta line in Fig.\ref{fig:arcLenvsAngles}(b) \& (c)). This is in keeping with the behaviour of the  PD, AD and LD muscles along which the tendons have been routed. The increase/decrease in sensor value in Fig.\ref{fig:arcLenvsAngles} is reflected in the change in colour on the surface plot. For the HAb/Ad movements as well, the observed sensor data from all 4 sensors conform to the behaviour of the muscles along which they were routed. The results of this movement are shown in the black lines in the 4 subplots of Fig.\ref{fig:arcLenvsAngles}. We can consider these results the validation of our proposed bio-inspired sensing concept. The red line corresponds to the arm in neutral/rest position.



Some inconsistencies in Fig.\ref{fig:arcLenvsAngles} are: 1). The red line in Fig.\ref{fig:arcLenvsAngles}(a) should have been a straight line since it represents the hand in neutral position. The curve is observed as it is an extrapolation by the ANN-fitting. The arm cannot reach $<10^{\circ}$ in that DoF due to the thickness of the suit, and the network, makes an estimation along that line in Fig.\ref{fig:arcLenvsAngles}(a). 2) Some non-monotonicity in the ANN-fitted surface is seen in the top-right corner of Fig.\ref{fig:arcLenvsAngles}(b)\&(d). This is again an extrapolation by the fitting, as that region is out of the shoulder's reachable workspace (blue dots absent).
 
 
%  In general, it can be observed that the values along this line stay steady at the base level (not zeroed here). There is no change in the sensor values along DoF-1 while keeping DoF-2 at $0^{\circ}$. The reason for this is that the arm is in  Gimbal lock in this pose. The slight drop in value in the sensor-\textbf{F} graph is due to the neural network based-fitting predicting a drop and not because of real values. Another observation in Fig.\ref{fig:arcLenvsAngles} is that the region where DoF-1 $<-45^{\circ}$ and DoF2 $>\approx30^{\circ}$ is not populated and this is because that region is out of the reachable workspace of the human arm. Additionally, the test subject expressed concern that the suit was restrictive especially when DoF-2 $>90^{\circ}$. We are exploring ways to reduce this restriction in the next design iteration.

% The results presented in Fig.\ref{fig:arcLenvsAngles} were partially observed in our simulation-based work \cite{Varghese2019BSN}, though the observed behaviour of simulated sensors was very different from the real sensors. The results obtained in Fig.\ref{fig:arcLenvsAngles} confirms our hypothesis in \cite{Varghese2019BSN}. We hypothesized that the reason for the non-monotonous nature of some sensors was due to the fact that in the simulations the virtual markers were fixed to a bone rather than the skin, and was not due to the choice of tendon-routing. As a result of the above, we had seen unexpected non-linear behaviour in the simulated sensor values during movements like horizontal A/A \textit{etc.}. This outcome has been disproved by the results presented in Fig.\ref{fig:arcLenvsAngles}. Though monotonous behaviour in the different sensors is observed for the different movements, some non-monotonous lines are present but this is due to the neural-network fitting and is not represented by the presence of real sensor values (\textit{e.g.} green line in Fig.\ref{fig:arcLenvsAngles}(d)).


\begin{figure}
\centering
\includegraphics[width = 1\linewidth]{RealvsVirtualComparison.png}
\caption{Comparison of real and virtual sensor performance I: a). Graphics of the top and front view of the pose of the upper-limb during the trial. b)-c). Real and virtual sensor-\textbf{F} \& \textbf{SF} values obtained during the trial. d). DoF-1 \& DoF-2 values during the trial. DoF-1 is held constant at a value while DoF-2 is changed from neutral to parallel to ground configuration.}
\label{fig:realVirtCompare}
\end{figure}


\subsection{Real v/s Virtual Sensing Analysis}
\label{subsec:realVsVirtRes}
To further study our sensing framework, virtual and real sensor values from a movement trial are compared in Fig. \ref{fig:realVirtCompare}\&\ref{fig:realVirtCompareII}. This analysis was done to understand the effects of compliance, friction and other non-linearities encountered by the real tendons vis-a-vis the unhindered virtual tendons. This sub-section presents the evolution of:
\begin{enumerate}
    \item real v/s virtual sensors w.r.t time (see Fig.\ref{fig:realVirtCompare}),
    \item real v/s virtual sensors w.r.t joint angles (see Fig.\ref{fig:realVirtCompareII}).
\end{enumerate}

  The OpenSim graphics in Fig.\ref{fig:realVirtCompare}(a) show the movement of the upper-limb in top and front/side view. The trial presented in Fig.\ref{fig:realVirtCompare} is detailed in Table \ref{tab:exp_mvmts} row 3 where the azimuth angle (DoF-1) is held at different constant values while varying the elevation angle (DoF-2). 5 movements (B-F) are performed in the trial where phase A, B and E represent neutral position, F/E and Ab/Ad respectively.

In Fig.\ref{fig:realVirtCompare}(b)\&(c), we observe that both real and virtual sensors follow the same trend lines for both sensors-\textbf{F}\&\textbf{SF}, and follow the behaviour of their associated muscles/synergies. For both sensors-\textbf{F}\&\textbf{SF} (see Fig.\ref{fig:realVirtCompare}(b)\&(c)), we see that the absolute peak value for both real and virtual sensors decrease with decreasing DoF-1 value. For sensor-\textbf{F}, the value goes almost to nil during Ab/Ad and changes direction when reverse F/E is performed, while for sensor-\textbf{SF}, the value follows the same trend as sensor-\textbf{F}, but goes to zero during reverse F/E movement. In sensor-\textbf{F}, there is some lag between the virtual and real sensor. This is observed because the tendon gets pinched near the axillary fossa (armpit) which increases friction and hinders movement. We intend to correct this in the next iteration by modifying the tendon-routing around the region. 
\begin{figure}
\centering
\includegraphics[width = 0.95\linewidth]{Hysteresis-SensorSF2.png}
\caption{Comparison of real and virtual sensor performance II: The graph shows the displacement of real (red) and virtual (blue) sensor-\textbf{SF} values against elevation angle during multiple F/E movements. This graph presents the hysteresis and error bands observed in both the real and virtual sensors.}
\label{fig:realVirtCompareII}
\end{figure}

The joint angle representation used for this work is in spherical coordinate system, \textit{i.e.} the representation adopted by the MS model \cite{Saul2015}. This representation has been used instead of quaternions as it is more intuitive and affords better visualization of results. The downside of this representation is the Gimbal lock problem, and is seen in the sharp change in DoF-1 value as the arm moves to the neutral position (see Fig.\ref{fig:realVirtCompare}(d)). We intend to switch to quaternion representation when using this sensing framework for feedback control.
% In the case of sensor-\textbf{SF} (see Fig.\ref{fig:realVirtCompare}(c)), the performance of the real sensor is closer to the virtual sensor-\textbf{SF}. Both real and virtual sensors retract during F/E movements, and the magnitude of the change in sensor values reduce as we go towards Ab/Ad movements and then becomes almost nil during reverse F/E movements. 

Fig.\ref{fig:realVirtCompareII} presents another comparison of the virtual and real sensor values when analyzed w.r.t joint angles. Fig.\ref{fig:realVirtCompareII} presents the evolution of sensor-\textbf{SF} value with changing elevation angle ($\phi$) during F/E movements. We can clearly see the existence of hysteresis behaviour in both the real and virtual sensors. In the case of virtual sensors, this behaviour is observed primarily due to the inherent soft nature of the neoprene base suit on which the markers are mounted. In the case of the real sensors, this behaviour is further exacerbated, because of the sensor limit imposed by the termination base (see Fig.\ref{fig:realVirtCompareII}). As previously mentioned, this was done for visual demonstrability of the concept, \textit{i.e.} to visualize tendon displacement as the shoulder moves (see accompanying video). The sensor is not able to recover completely from the imposed sensor limit as we have additional non-linearities introduced by: 1). the friction between tendons and the routing elements, tendon-sheaths, \textit{etc.}, and 2). the local pulling (compliance) experienced at the termination elements due to the spring force of the sensor transmitted by the tendon.  It is predominantly due to the imposed sensor limit that the tendon experiences a small permanent deformation at the end of sequence of F/E movements. Similar behaviour is observed in other movements as well. The small error band of observed real/virtual sensor values over repeated movements (see Fig.\ref{fig:realVirtCompareII}) demonstrates the repeatability of the framework. 
% The error band increases in width as we get closer to the rest/neutral position, due to reduced rate of change of sensor value close to the neutral position (see magenta line in Fig.\ref{fig:arcLenvsAngles}(b)). 
We intend to address the friction- and compliance-related shortcomings with adequate design countermeasures in the next version of the suit.     

% In the current prototype, the total travel for each sensor is limited between the string-pot and the tendon-sheath termination base, and it is reached in the case of tendon-\textbf{SF} (see Fig.\ref{fig:realVirtCompare} \& \ref{fig:realVirtCompareII}). As previously mentioned, this was done for visual demonstrability of the concept, \textit{i.e.} to visualize tendon displacement as the shoulder moves (see attached video). This will be replaced with a tendon-sheath in the next iteration. 

% But, we also observe that the real sensor lags behind the virtual sensor when the DoF-2 value increases above a certain value. During the experiments, we observed that as the arm moves up, the section of the tendon at the junction between the arm and the trunk gets pinched by skin folds generated above a certain angle, and this leads to an increase in friction. This added friction isn't instantaneously compensated by the spring in the string-pot and results in the lag between the real and virtual sensors. We are working on a solution to circumvent this problem. 

\begin{figure}
\centering
\includegraphics[width = \linewidth]{MappingPerformance2.png}
\caption{$\textbf{S}\mapsto\textbf{q}$ Mapping Performance: RMSE for DoF-1 \& DoF-2 for an ANN with 1 hidden layer of 25 neurons. The sensor combination performing the best is encapsulated in the black box. The results for IMU-based solution is shown with orange (DoF-1) and green (DoF-2) bars.}
\label{fig:mapPerform}
\end{figure}

  
% In the case of sensor-\textbf{SF}, a limitation in the tendon travel limit is imposed by the tendon-sheath termination base (see Fig.\ref{fig:hardwareModel}) .  In the case of sensor-\textbf{SF}, we can see this limit being hit in Fig.\ref{fig:realVirtCompare}(c). Due to this limit being hit as the sensor value decreases, the tendon slackens at the top of the string-pot. Now when the tendon is being pulled back, it first needs to recover from the slack and it is this recovery that could result in a drift between the real and virtual values. 
% not be present in the next iteration of the suit. In the next iteration of the suit, we intend to have the Bowden-cable tendon-sheath all the way to the top of the string-pot thereby allowing full range of travel for the sensor. 
% Apart from this, we also need to improve friction management as more drift is encountered when the tendon slackens and depends on the string-pot's spring to be maintained taut (see Fig.\ref{fig:realVirtCompare}(c)). Similar behaviour is also observed in the case of sensors-\textbf{F},\textbf{SR} and \textbf{R}. This behaviour looks very similar to a hysteresis curve when plotted against joint angles, and we are working towards minimizing this non-linearity.


% From Fig.\ref{fig:realVirtCompare}(d), we can see a limitation in our derivation of the joint angles. This limitation is in the joint angle convention adopted in the OpenSim musculoskeletal model by Saul \textit{et al.}\cite{Saul2015}. It can be seen that the Gimbal lock problem is encountered (see Fig.\ref{fig:realVirtCompare}(d)). When the upper-limb gets close to the neutral position (DoF-2 $\approx  <25^{\circ}$), there is a sharp change in DoF-1 value. This leads to the problem that for the same sensor and DoF-2 value, the DoF-1 value can assume a very large range of values. This is shown in Fig.\ref{fig:realVirtCompare}(d) with the red-boundary boxes. This was a limitation that did not surface during our simulation-based work in \cite{Varghese2019BSN}, as we were doing forward kinematics to generate data (instead of inverse kinematics as is the case here), and also had the option to generate a huge amount of data in the entire workspace to learn the mapping. This is not possible in the case with human subjects. We intend to investigate quaternions and other representation to represent the shoulder joint angles in the future and overcome this limitation of our work. 



\subsection{Sensor-to-Joint Space Mapping Performance}
\label{subsec:NNMapRes}
% The Gimbal lock shortcoming discussed in the previous sub-section limits the data that can be used for training our ANN to learn the sensor-to-joint space mapping. To derive the sensor-to-joint space mapping, we created two ANNs - one that was trained on all the sensor and corresponding joint angle data, and a second network which was trained on data that did not have any data in the Gimbal lock regions. To get the data for the second mapping, all data with DoF-2 $< 30^{\circ}$ were discarded. The performance of both networks for both DoF-1 \& DoF-2 can be seen in Fig.\ref{fig:mapPerform}. 
This sub-section discusses the performance of the ANN-based $\textbf{S}\mapsto\textbf{q}$ mapping as presented in Fig.\ref{fig:mapPerform}.  Fig.\ref{fig:mapPerform} shows the performance of the $\textbf{S}\mapsto\textbf{q}$ mapping learned using different networks and varying number of virtual sensors as inputs to the network. The network using all the 4 sensors performed the best followed by comparable performances observed by different combinations of the three sensors. This is followed by the performances of different pairs of sensors. This behaviour is analogous to the behaviour observed in \cite{Budhota2017} where 4 muscle synergies accounted for more than 90\% of the variance in shoulder movements followed by comparable performance by 3 synergies and reduced performance by 2 synergies. In Fig.\ref{fig:mapPerform}, the anomaly is the combination of sensors-\textbf{F}\&\textbf{R}, which shows a significantly high RMS error. This is observed because sensors-\textbf{F}\&\textbf{R} are almost an agonist-antagonist pair, thereby bringing in very similar contributions to the $\textbf{S}\mapsto\textbf{q}$ map.
%  On comparing the data with and without the data experiencing Gimbal lock, we can easily see that the network trained without the Gimbal lock data outperforms the network trained on all the data. The Gimbal lock affects both DoF-1 and DoF-2 fitting, but the effect on DoF-2 is marginal and this is as expected, whereas the effect of DoF-2 is more profound. 
 We can see that an RMSE of $5.43^{\circ}$ in DoF-1 and $3.65^{\circ}$ in DoF-2 was achieved with a network having 25 neurons in the hidden layer and an input from all 4 sensors.  These results are promising as we have used a vanilla ANN-based fitting and have achieved RMSE comparable with state-of-the-art IMU-based sensing solutions in DoF-2 \cite{Aslani2018}. 
 
 As mentioned earlier, the advantage of our system over state-of-the-art IMU-based solutions is the ability to use the system in space environments as well, where IMUs could malfunction. From the size perspective, both systems can be very low-profile over the limbs and only require electronics that can be placed inside a backpack. Additionally, another advantage of this framework is the ability to use the sensing tendons as a benchmark for tendons in the actuation system for compensating backlash.  Due to the observed hysteresis (see Fig.\ref{fig:realVirtCompareII}), we hypothesize that the results of $\textbf{S}\mapsto\textbf{q}$ mapping can be further improved with history-based learning and statistical sensor-fusion methods like Recurrent Neural Networks (RNNs), Long Short-Term Memory (LSTM) networks and different Kalman filters.
%  In the future, we intend to explore more sophisticated statistical and learning based methods like Kalman filters, autoencoders to model hysteresis, and Long Short-Term Memory networks. 
%  The performance of the network trained on all data is not acceptable in the present state (especially for DoF-1) and we think that this problem can be solved by using quaternions instead of the current representation. In conclusion, we have demonstrated the possibility of using the proposed sensing framework along with the sensor mapping to good enough sensor performance to allow gross motor control for the exosuit.

